Planar Embeddings with Small and Uniform Faces

Motivated by finding planar embeddings that lead to drawings with favorable aesthetics, we study the problems MINMAXFACE and UNIFORMFACES of embedding a given biconnected multi-graph such that the largest face is as small as possible and such that all faces have the same size, respectively. We prove a complexity dichotomy for MINMAXFACE and show that deciding whether the maximum is at most $k$ is polynomial-time solvable for $k \leq 4$ and NP-complete for $k \geq 5$. Further, we give a 6-approximation for minimizing the maximum face in a planar embedding. For UNIFORMFACES, we show that the problem is NP-complete for odd $k \geq 7$ and even $k \geq 10$. Moreover, we characterize the biconnected planar multi-graphs admitting 3- and 4-uniform embeddings (in a $k$-uniform embedding all faces have size $k$) and give an efficient algorithm for testing the existence of a 6-uniform embedding.

==> makefile <==
finalname = arXiv

psfiles = \


pdf:
	pdflatex $(finalname).tex



startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.out
	rm -f *.backup
	rm -f *.pdf
	rm -f *.gz
	rm -f *.bbl
	rm -rf _*
	rm -f *.fmt

bib: 
	pdflatex $(finalname).tex
	bibtex $(finalname)
	pdflatex $(finalname).tex
	pdflatex $(finalname).tex

ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o



print: ps
	lpr -Ppolaris -h $(finalname).ps

